Discovering Partially Known Ordinary Differential Equations: a Case Study on the Chemical Kinetics of Cellulose Degradation

The degree of polymerization (DP) is one of the methods for estimating the aging of the polymer based insulation systems, such as cellulose insulation in power components. The main degradation mechanisms in polymers are hydrolysis, pyrolysis, and oxidation. These mechanisms combined cause a reduction of the DP. However, the data availability for these types of problems is usually scarce. This study analyzes insulation aging using cellulose degradation data from power transformers. The aging problem for the cellulose immersed in mineral oil inside power transformers is modeled with ordinary differential equations (ODEs). We recover the governing equations of the degradation system using Physics-Informed Neural Networks (PINNs) and symbolic regression. We apply PINNs to discover the Arrhenius equation's unknown parameters in the Ekenstam ODE describing cellulose contamination content and the material aging process related to temperature for synthetic data and real DP values. A modification of the Ekenstam ODE is given by Emsley's system of ODEs, where the rate constant expressed by the Arrhenius equation decreases in time with the new formulation. We use PINNs and symbolic regression to recover the functional form of one of the ODEs of the system and to identify an unknown parameter.

==> Nomenclature.tex <==
\section*{Nomenclature}

\begin{table}[]
    %\centering
    \begin{tabular}{lll}
$\lambda_u$ & & is the weight for the data loss function\\
$\lambda_f$ & &  is the weight for residual loss function\\

$n$ && is a reference number for input datapoint $n \in N$ \\
$N$ && is the size of an input dataset\\
$N_u$ && size of the input dataset for $MSE_u$\\
$N_f$ && size of the input dataset for $MSE_f$\\
$T$ && is the reference temperature \\
$\hat{T}$ && is the output temperature \\


    $f$ && \\
    
      
      MSE && Mean square error \\


      
      $n_{in}$   && number of input units  \\
      $n_{out}$ && number of output units \\

      $u$ && \\
    $W$ && weights \\
    $X^n$ && is the $n$-th input data point for MSE \\
    $\rho$ && is the density [kg/m$^3$] \\
    $c_p$ && is the specific heat capacity [J/kg$\cdot$K]\\
    $t$ && is the time reference point \\
    $x$ && is the spatial reference point \\
    $k$ && is the thermal conductivity [W/m$\cdot$K] \\
    $K$ && is the load factor [p.u.]\\
    $P_0$ && is the no-load loss [W]\\
    $P_K$ && is the load loss \\
    $h$ && is the convective heat transfer coefficient [W/m$^2 \cdot$K]\\
    %$\Delta_x$ && is a Laplacian \\
    $l$ && denote the layer number, $l \in L$\\ 
    $L$ && is the total number of layers \\
    $\sigma$ && is the neural network activation function \\
    $q$ && is \\
    $\hat{Y}$ && \\
    $b$ && denotes biases \\
    $MAE$ && is the Mean Absolute Error \\
    $j$ && is the \\
    $i$ && \\
    $\varepsilon$ && is \\
    
    \end{tabular}
   % \caption{Caption}
    \label{tab:my_label}
\end{table}
